InterHandGen: Two-Hand Interaction Generation via Cascaded Reverse Diffusion

We present InterHandGen, a novel framework that learns the generative prior of two-hand interaction. Sampling from our model yields plausible and diverse two-hand shapes in close interaction with or without an object. Our prior can be incorporated into any optimization or learning methods to reduce ambiguity in an ill-posed setup. Our key observation is that directly modeling the joint distribution of multiple instances imposes high learning complexity due to its combinatorial nature. Thus, we propose to decompose the modeling of joint distribution into the modeling of factored unconditional and conditional single instance distribution. In particular, we introduce a diffusion model that learns the single-hand distribution unconditional and conditional to another hand via conditioning dropout. For sampling, we combine anti-penetration and classifier-free guidance to enable plausible generation. Furthermore, we establish the rigorous evaluation protocol of two-hand synthesis, where our method significantly outperforms baseline generative models in terms of plausibility and diversity. We also demonstrate that our diffusion prior can boost the performance of two-hand reconstruction from monocular in-the-wild images, achieving new state-of-the-art accuracy.

==> tab/arctic_feature.tex <==
\begin{table*}[!t]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{?}}
\label{table:interhand_feature}

\begin{tabularx}{2\columnwidth}{>{\centering}m{3.7cm}|Y|Y|Y|Y|Y}
\toprule
Method & FID $\downarrow$ & KID $\downarrow$ & Diversity $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$\\
\midrule
CVAE~\cite{} & ? & ? & ? & ? & ? \\
BUDDI~\cite{muller2023generative} & 36.13 & 0.28 & 6.83 & 0.26 & 0.31 \\
Ours w/o Decomp. & 32.41 & 0.22 & 7.24 & 0.38 & 0.63 \\
Ours w/o Cond. Dropout  & 26.01 & 0.52 & 6.69 & \textbf{0.78} & 0.61 \\
\textbf{Ours} & \textbf{20.07} & \textbf{0.10} & \textbf{7.43} & 0.73 & \textbf{0.64} \\
\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table*}

==> tab/interhand_feature.tex <==
\begin{table*}[!t]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{?}}
\label{table:interhand_feature}

\begin{tabularx}{2\columnwidth}{>{\centering}m{3.7cm}|Y|Y|Y|Y|Y}
\toprule
Method & FID $\downarrow$ & KID ($\times 10^{-2}$) $\downarrow$ & Diversity $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$\\
\midrule
VAE~\cite{zuo2023reconstructing} & 8.18 & 6.23 & 2.32 & 0.55 & 0.02 \\
BUDDI~\cite{muller2023generative} & 3.48 & 4.10 & 2.71 & 0.56 & 0.47 \\
Ours w/o Decomp.  & 2.09 & 0.75 & 2.46 & 0.86 & 0.35 \\
Ours w/o Cond. Dropout  & 1.32 & 0.46 & 2.34 & \textbf{0.92} & 0.42 \\
\textbf{Ours} & \textbf{0.71} & \textbf{0.36} & \textbf{3.33} & 0.86 & \textbf{0.85} \\
\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table*}

==> tab/interhand_mano.tex <==
\begin{table*}[!t]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{?}}
\label{table:interhand_mano}

\begin{tabularx}{2\columnwidth}{>{\centering}m{3.7cm}|Y|Y|Y|Y|Y}
\toprule
Method & FID $\downarrow$ & KID $\downarrow$ & Diversity $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$\\
\midrule
VAE~\cite{zuo2023reconstructing} & 58.32 & 1.04 & 9.95 & 0.73 & 0.02 \\
BUDDI~\cite{muller2023generative} & 28.17 & 0.74 & 10.55 & 0.69 & 0.45 \\
Ours w/o Decomp.  & 41.78 & 0.98 & 10.27 & 0.75 & 0.30 \\
Ours w/o Cond. Dropout  & 19.53 & 0.59 & 10.04 & \textbf{0.78} & 0.55 \\
\textbf{Ours} & \textbf{11.68} & \textbf{0.22} & \textbf{11.91} & 0.75 & \textbf{0.83} \\
\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table*}

==> tab/supp_diversity.tex <==
\begin{table}[!h]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}

\caption{\textbf{.}} 
\label{table:supp_diversity}
\vspace{-0.5\baselineskip}
\begin{tabularx}{\columnwidth}{>{\centering}m{3cm}|Y|Y}
\toprule
Method & Ours & Ours w/ Aug. \\
\midrule 
Diversity $\uparrow$ & 3.59 & \textbf{4.39} \\
\bottomrule
\end{tabularx}}
\end{table}

==> tab/supp_layer_conf.tex <==
\begin{table*}[h]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{Layer configurations of our diffusion model $D_{\theta}$.}
\vspace{-0.5\baselineskip}
\label{table:layer_configuration}

\begin{tabularx}{\textwidth}{>{\centering}m{2.6cm}|>{\centering}m{8.4cm}|Y}
\toprule
 & Layer Description & Output Dimension \\
\midrule
TCNN-1 & (Temporal conv., filter size 3, 96 features, stride 2) & $J \times 96 \times 8$ \\
TCNN-2 & (Temporal conv., filter size 3, 64 features, stride 2) & $J \times 64 \times 3$ \\
TCNN-3 & (Temporal conv., filter size 3, 64 features, stride 1) & $J \times 64 \times 1$ \\
\midrule
MLP-1 & (Linear, 128 features) & $J \times 128$ \\
MLP-2 & (Linear, 64 features) & $J \times 64$ \\
MLP-3 & (Linear, 14 ($= 6N+3$) features) & $J \times 14 \, (= 6N+3)$ \\
\bottomrule
\end{tabularx}
}
\end{table*}

==> tab/supp_mano_feature_comparisons.tex <==
\begin{table*}[!t]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Quantitative evaluations of two-hand interaction synthesis using our two-hand PointNet++~\cite{qi2017pointnet++} features and MANO~\cite{romero2017embodied} parameter features.} \textbf{Bold} indicates the best scores, and \underline{underline} indicates the second best scores. The experimental setting is the same as in Section~\ref{subsec:two-hand} in the main paper.}

\label{table:supp_mano_feature_comparisons}

\begin{subtable}[t]{\textwidth}
\caption{\textbf{Comparisons on two-hand interaction generation (Section~\ref{subsec:two-hand})}.}
\begin{tabularx}{\textwidth}{>{\centering}m{3.4cm}|Y|Y|Y|Y|Y}
\toprule
Method & FHID $\downarrow$ & KHID \tiny{($\times 10^{-2}$)} \normalsize{$\downarrow$} & Diversity $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ \normalsize{$\downarrow$} \\
\midrule
VAE~\cite{zuo2023reconstructing} & 8.18 & 6.23 & 2.32 & 0.55 & 0.02 \\
BUDDI*~\cite{muller2023generative} & 3.48 & 4.10 & \underline{2.71} & 0.56 & \underline{0.47} \\
Ours w/o Decomposition  & 2.09 & 0.75 & 2.34 & \underline{0.86} & 0.35 \\
Ours w/o Shared Network  & \underline{1.32} & \underline{0.46} & 2.46 & \textbf{0.92} & 0.42 \\
\textbf{Ours} & \textbf{1.00} & \textbf{0.15} & \textbf{3.59} & \underline{0.86} & \textbf{0.85} \\
\bottomrule
\end{tabularx}
\label{subtable:two-hand}
\end{subtable}
\vspace{-0.4\baselineskip}

% this table is incomplete yet 
\begin{subtable}[t]{\textwidth}
\caption{\textbf{Comparisons on object-conditioned two-hand interaction generation (Section~\ref{subsec:two-hand-object})}.}
\begin{tabularx}{\textwidth}{>{\centering}m{3.4cm}|Y|Y|Y|Y|Y}
\toprule
Method & FHID $\downarrow$ & KHID \normalsize{$\downarrow$} & Diversity $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ \\
\midrule
VAE~\cite{zuo2023reconstructing} & 58.32 & 1.04 & 9.95 & 0.73 & 0.02 \\
BUDDI*~\cite{muller2023generative} & 28.17 & 0.74 & 10.55 & 0.69 & 0.45 \\
Ours w/o Decomposition & 19.84 & 1.18 & 6.28 & 0.40 & \textbf{0.67} \\
Ours w/o Shared Network & 
\underline{17.00} & \underline{0.97} & 6.15 & \textbf{0.74} & \underline{0.63} \\
\textbf{Ours} & \textbf{12.91} & \textbf{0.55} & \textbf{6.77} & \underline{0.71} & \textbf{0.67} \\
\bottomrule
\end{tabularx}
\label{subtable:two-hand-object}
\end{subtable}
}
%\vspace{-0.5\baselineskip}
\end{table*}

